Perception-Oriented Video Frame Interpolation via Asymmetric Blending

Previous methods for Video Frame Interpolation (VFI) have encountered challenges, notably the manifestation of blur and ghosting effects. These issues can be traced back to two pivotal factors: unavoidable motion errors and misalignment in supervision. In practice, motion estimates often prove to be error-prone, resulting in misaligned features. Furthermore, the reconstruction loss tends to bring blurry results, particularly in misaligned regions. To mitigate these challenges, we propose a new paradigm called PerVFI (Perception-oriented Video Frame Interpolation). Our approach incorporates an Asymmetric Synergistic Blending module (ASB) that utilizes features from both sides to synergistically blend intermediate features. One reference frame emphasizes primary content, while the other contributes complementary information. To impose a stringent constraint on the blending process, we introduce a self-learned sparse quasi-binary mask which effectively mitigates ghosting and blur artifacts in the output. Additionally, we employ a normalizing flow-based generator and utilize the negative log-likelihood loss to learn the conditional distribution of the output, which further facilitates the generation of clear and fine details. Experimental results validate the superiority of PerVFI, demonstrating significant improvements in perceptual quality compared to existing methods. Codes are available at \url{https://github.com/mulns/PerVFI}

==> Tables/assets.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{p{0.13\linewidth}|p{0.55\linewidth}|p{0.25\linewidth}}
\toprule
Dataset & URL & License / Terms of Use \\
\midrule
Vimeo90K~\cite{toflow} & \url{http://toflow.csail.mit.edu} & MIT license. \\ \midrule
DAVIS~\cite{davis} & \url{https://davischallenge.org} & BSD license. \\ \midrule
Sintel~\cite{sintel} & \url{http://sintel.is.tue.mpg.de} & Available for research use. \\ \midrule
Xiph~\cite{softmaxsplat2020} & \url{https://media.xiph.org/video/derf} & Available for research use. \\ \midrule
Adobe240~\cite{adobe240} & \url{https://www.cs.ubc.ca/labs/imager/tr/2017/DeepVideoDeblurring/} & MIT License. \\ \midrule
UCF101~\cite{ucf101} & \url{https://www.crcv.ucf.edu/data/UCF101.php} & Available for research use. \\ \midrule
Middlebury~\cite{middlebury} & \url{https://vision.middlebury.edu/flow/data/} & Available for research use. \\
\bottomrule
\end{tabular}
\vspace{0.1in}
\caption{Attribution of datasets used in this work.}
\label{tab:data}
\end{table*}

\begin{table*}[t]
\centering
\begin{tabular}{p{0.13\linewidth}|p{0.55\linewidth}|p{0.25\linewidth}}
\toprule
Method & URL & License / Terms of Use \\
\midrule
EDSC~\cite{edsc2020} & \url{https://github.com/Xianhang/EDSC-pytorch} & Available for research use. \\ \midrule
XVFI~\cite{xvfi2021} & \url{https://github.com/JihyongOh/XVFI} & Available for research use. \\ \midrule
RIFE~\cite{huang2020rife}& \url{https://github.com/megvii-research/ECCV2022-RIFE} & MIT license. \\ \midrule
EBME~\cite{Jin_2023_WACV} & \url{https://github.com/srcn-ivl/EBME} & Apache-2.0 License \\ \midrule
STMFNet~\cite{Danier_2022_CVPR} & \url{https://github.com/danielism97/ST-MFNet} & MIT license. \\ \midrule
RAFT~\cite{raft} & \url{https://github.com/princeton-vl/RAFT} & BSD License. \\ \midrule
VFIFormer~\cite{vfiformer} & \url{https://github.com/dvlab-research/VFIformer} & MIT license. \\ \midrule
EMA-VFI~\cite{zhang2023extracting} & \url{https://github.com/MCG-NJU/EMA-VFI/tree/main} & Apache-2.0 License. \\ \midrule
RAFT~\cite{raft} & \url{https://github.com/princeton-vl/RAFT} & BSD License. \\ \midrule
GMA~\cite{gma} & \url{https://github.com/zacjiang/GMA} & Available for research use. \\ \midrule
GMFlow~\cite{gmflow} & \url{https://github.com/haofeixu/gmflow} & Apache-2.0 License. \\ 

\bottomrule
\end{tabular}
\vspace{0.1in}
\caption{Attribution of code assets used in this work.}
\label{tab:code}
\end{table*}

==> Tables/full.tex <==

\begin{table*}[htbp]
  \centering
  \caption{Performance comparison of VFI methods on Middlebury~\cite{middlebury}, Vimeo-90K~\cite{vimeo}, and UCF101~\cite{ucf101} datasets. The best values are highlighted in \textbf{\textcolor{red}{red}}. The STMFNet does not support triplet datasets.}
  \label{tab:other-dst}
  \begin{tabular}{lccc|ccc|ccc}
    \toprule
    & \multicolumn{3}{c}{Middlebury} & \multicolumn{3}{c}{Vimeo-90K} & \multicolumn{3}{c}{UCF101} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
    Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
    \midrule
    EDSC~\cite{edsc2020} & 39.540 & 0.979 & 0.014 & 34.857 & 0.961 & 0.027 & 33.392 & 0.954 & 0.030 \\
    RIFE~\cite{huang2020rife} & 37.115 & 0.963 & 0.013 & 34.164 & 0.955 & 0.020 & 33.006 & 0.950 & 0.027 \\
    EBME~\cite{Jin_2023_WACV} & 39.551 & 0.977 & 0.011 & 35.422 & 0.965 & 0.022 & 33.468 & 0.954 & 0.029 \\
    VFIFormer~\cite{vfiformer} & \textbf{\color{red}40.586} & \textbf{\color{red}0.982} & 0.011 & \textbf{\color{red}36.384} & \textbf{\color{red}0.971} & 0.021 & 33.571 & 0.955 & 0.031 \\
    STMFNet~\cite{Danier_2022_CVPR} & - & - & - & - & - & - & \textbf{\color{red}34.161} & \textbf{\color{red}0.958} & 0.031 \\
    EMA-VFI~\cite{zhang2023extracting} & 37.364 & 0.966 &  0.020 & 36.339 & 0.967 & 0.026 & 33.591 & 0.956 & 0.031 \\
    PerVFI (ours) & 38.005 & 0.971 & \textbf{\red{0.009}} & 34.141 & 0.958 & \textbf{\color{red}0.018} & 32.295 & 0.945 & \textbf{\color{red}0.026} \\
    \bottomrule
  \end{tabular}
\end{table*}


\begin{table*}[tbp]
  \centering
  \caption{Performance comparison of VFI algorithms on DAVIS-2017~\cite{davis}. The best values are highlighted in \textbf{\textcolor{red}{red}}. ``Out of Memory” is denoted as “OOM”.}
  \label{tab:davis}
  \vspace{-5pt}
  \begin{adjustbox}{max width=\textwidth}
  \begin{tabular}{lcccccccccc} % cccccccccc llllllllll
    \toprule
    {} & \multicolumn{5}{c}{{DAVIS (480P)}} & \multicolumn{5}{c}{{DAVIS (1080P)}} \\
    \cmidrule(lr){2-6} \cmidrule(lr){7-11}
    & {PSNR}$\uparrow$ & SSIM $\uparrow$ & {LPIPS}$\downarrow$ & {FloLPIPS$\downarrow$} & {VFIPS$\uparrow$} & {PSNR$\uparrow$} & SSIM$\uparrow$ & {LPIPS}$\downarrow$ & {FloLPIPS}$\downarrow$ & {VFIPS}$\uparrow$ \\
    \midrule
    EDSC~\cite{cheng2021multiple} & 26.52 & 0.784 & 0.132 & 0.093 & 72.62 & 24.54 & 0.768 & 0.205 & 0.138 & 51.05 \\
    XVFI~\cite{sim2021xvfi} & 26.42 & 0.79 & 0.120 & 0.087 & 74.76 & 26.03 & 0.812 & 0.145 & 0.109 & 62.17\\
    RIFE~\cite{huang2020rife} & 26.97 & 0.807 & {0.085} & {0.063} & {80.19} & 25.89 & 0.803 & {0.134} & {0.097} & {62.56}\\
    EBME~\cite{Jin_2023_WACV} & {27.27} & 0.811 & 0.112 & 0.081 & 77.43 & 25.09 & 0.793 & 0.194 & 0.132 & 53.82\\
    STMFNet~\cite{Danier_2022_CVPR} & 28.55 & 0.850 & 0.121 & 0.086 & 77.38 & 27.43 & 0.844 & 0.178 & 0.119 & 60.25\\
    VFIFormer~\cite{vfiformer} & 27.34 & 0.814 &  0.124 &  0.140 &  76.57     & OOM & OOM & OOM & OOM & OOM \\
    EMA-VFI~\cite{zhang2023extracting} & {\bf\color{red}28.83} & {\bf\color{red}0.856} &  0.127 &  0.125 &  78.79 & {\bf\color{red}27.61} & {\bf\color{red}0.846} &  0.203 &  0.171 &  58.94 \\
    PerVFI & 27.16&     0.816&      \textbf{\textcolor{red}{0.075}} &     \textbf{\textcolor{red}{0.056}}&      \textbf{\textcolor{red}{83.30}} & 26.34 & 0.816 & \textbf{\textcolor{red}{0.112}} & \textbf{\textcolor{red}{0.085}} & \textbf{\textcolor{red}{68.47}}  \\
    \bottomrule
  \end{tabular}
  \end{adjustbox}
\end{table*}


\begin{table}[t]
  \centering
  \caption{Performance comparison of VFI algorithms on Adobe240~\cite{adobe240}. The best values are highlighted in \textbf{\textcolor{red}{red}}.}
  \label{tab:adobe}
  \begin{adjustbox}{max width=\linewidth}
  \begin{tabular}{lccccc} % cccccccccc llllllllll
    \toprule
    {} & \multicolumn{5}{c}{{Adobe240}} \\
    \cmidrule(lr){2-6}
    & {PSNR}$\uparrow$ & SSIM $\uparrow$ & {LPIPS}$\downarrow$ & {FloLPIPS$\downarrow$} & {VFIPS$\uparrow$} \\
    \midrule
    
        EDSC~\cite{cheng2021multiple} & 41.50 & 0.984 & 0.010 & 0.005 & 108.2 \\
        XVFI~\cite{sim2021xvfi} & 38.48 & 0.976 & 0.032 & 0.014 & 105.5 \\
        RIFE~\cite{huang2020rife} & 40.19 & 0.981 & 0.011 & 0.006 & 107.5 \\
        EBME~\cite{Jin_2023_WACV} & 41.34 & 0.984 & 0.011 & 0.006 & 108.7 \\
        STMFNet~\cite{Danier_2022_CVPR} & \textbf{\color{red}41.51} & 0.980 & 0.012 & 0.006 & 108.3 \\
        EMA-VFI~\cite{zhang2023extracting} & 41.50 & \textbf{\color{red}0.985} & 0.012 & 0.006 & 108.3 \\
        
        PerVFI & 40.51 & 0.980 & \textbf{\color{red}0.006} & \textbf{\color{red}0.004} & \textbf{\color{red}109.2} \\

    \bottomrule
  \end{tabular}
  \end{adjustbox}
\end{table}


\begin{table*}[t]
  \centering
  \caption{Performance comparison of VFI algorithms on Xiph2K and Xiph4K~\cite{softmaxsplat2020}. The best values are highlighted in \textbf{\textcolor{red}{red}}}
  \label{tab:xiph}
  \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{lcccccccccc}
      \toprule
      & \multicolumn{5}{c}{Xiph - 2K} & \multicolumn{5}{c}{Xiph - ``4K''} \\
      \cmidrule(lr){2-6} \cmidrule(lr){7-11}
      & {PSNR}$\uparrow$ & SSIM $\uparrow$ & {LPIPS}$\downarrow$ & {FloLPIPS$\downarrow$} & {VFIPS$\uparrow$} & {PSNR}$\uparrow$ & SSIM $\uparrow$ & {LPIPS}$\downarrow$ & {FloLPIPS$\downarrow$} & {VFIPS$\uparrow$} \\
      \midrule
  
      EDSC~\cite{cheng2021multiple} & 34.80 & 0.932 & 0.085 & 0.072 & 64.73 & 31.81 & 0.881 & 0.177 & 0.120 & 51.24 \\
      XVFI~\cite{sim2021xvfi} & 34.63 & 0.925 & 0.071 & 0.051 & 63.37 & 32.74 & 0.884 & 0.123 & 0.076 & 52.98 \\
      RIFE~\cite{huang2020rife} & 35.41 & 0.927 & 0.041 & 0.050 & 65.26 & 33.10 & 0.881 & 0.099 & 0.067 & 54.31 \\
      EBME~\cite{Jin_2023_WACV} & 36.01 & 0.938 & 0.091 & 0.059 & 65.33 & 32.96 & 0.896 & 0.204 & 0.114 & 52.79 \\
      STMFNet~\cite{Danier_2022_CVPR} & 37.11 & 0.946 & 0.110 & 0.063 & 65.19 & 34.80 & \textbf{\color{red}0.912} & 0.245 & 0.128 & 53.33 \\
      EMA-VFI~\cite{zhang2023extracting} & \textbf{\color{red}37.18} & \textbf{\color{red}0.946} & 0.110 & 0.081 & 65.12 & \textbf{\color{red}34.85} & 0.911 & 0.241 & 0.114 & 53.57 \\
      PerVFI & 34.95 & 0.927 & \textbf{\color{red}0.037} & \textbf{\color{red}0.033} & \textbf{\color{red}65.39} & 32.48 & 0.879 & \textbf{\color{red}0.084} & \textbf{\color{red}0.056} & \textbf{\color{red}54.52} \\
  
      \bottomrule
    \end{tabular}
  \end{adjustbox}
\end{table*}





\begin{table*}[tbp]
  \centering
  \caption{Quantitative comparison for 4$\times$ interpolation with extreme large motions. The best performing values are highlighted in \textbf{\textcolor{red}{red}}.}
  \label{tab:x4}
  \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{lcccccccccc}
      \toprule
    {} & \multicolumn{5}{c}{{Xiph - 2K - 4$\times$}} & \multicolumn{5}{c}{{Xiph - ``4K'' - 4$\times$}} \\
    \cmidrule(lr){2-6} \cmidrule(lr){7-11}
    & {PSNR}$\uparrow$ & SSIM $\uparrow$ & {LPIPS}$\downarrow$ & {FloLPIPS$\downarrow$} & {VFIPS$\uparrow$} & {PSNR$\uparrow$} & SSIM$\uparrow$ & {LPIPS}$\downarrow$ & {FloLPIPS}$\downarrow$ & {VFIPS}$\uparrow$ \\
    \midrule
    XVFI~\cite{xvfi2021} & 30.67 & 0.888 & 0.085 & 0.131 & 55.66 & 28.91 & 0.840 & 0.146 & 0.169 & 40.57 \\
    EBME~\cite{Jin_2023_WACV} & 30.00 & 0.893 & 0.122 & 0.163 & 54.04 & 26.96 & 0.828 & 0.258 & 0.683 & 29.84 \\
    EMA-VFI~\cite{zhang2023extracting} & {\bf\color{red}33.63} & {\bf\color{red}0.927} & 0.127 & 0.108 & 58.62 & {\bf\color{red}31.12} & {\bf\color{red}0.882} & 0.262 & 0.683 & 42.17 \\
    PerVFI & 30.72 & 0.891 & {\bf\color{red}0.054} & {\bf\color{red}0.101} & {\bf\color{red}58.84} & 28.66 & 0.838 & {\bf\color{red}0.109} & {\bf\color{red}0.680} & {\bf\color{red}43.52} \\
    \bottomrule
    \end{tabular}
  \end{adjustbox}
\end{table*}



\begin{table}[tbp]
  \centering
  \caption{Performance comparison of different optical flow estimators in PerVFI. The best performing values are highlighted in \textbf{\textcolor{red}{red}}, while the second-best values are in \underline{\textcolor{blue}{blue}}. It is important to note that \textbf{our PerVFI model is initially trained using optical flows obtained from RAFT~\cite{raft} and GMFlow~\cite{gmflow} networks. By replacing the optical flow estimator with GMA~\cite{gma} during the reference phase, we observe that our model achieves comparable performance}. This finding highlights the generalization ability of our method, as it demonstrates the capacity to adapt to different optical flow estimators without sacrificing performance. The consistent performance across different estimators further supports the robustness and effectiveness of our PerVFI framework.}
  \label{tab:optical-flows}
  \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{lccccc} % cccccccccc llllllllll
      \toprule
      {} & \multicolumn{5}{c}{{DAVIS (480P)}} \\
      \cmidrule(lr){2-6}
      & {PSNR}$\uparrow$ & SSIM $\uparrow$ & {LPIPS}$\downarrow$ & {FloLPIPS$\downarrow$} & {VFIPS$\uparrow$} \\
      \midrule
      RAFT-small+PerVFI & 26.84 & 0.812 & 0.080 & 0.062 & 81.15 \\
      GMFlow+PerVFI & 27.13 & \underline{\textcolor{blue}{0.815}} & 0.077 & 0.058 & 82.98 \\
      GMA+PerVFI & \textbf{\textcolor{red}{27.19}} & \textbf{\textcolor{red}{0.816}} & \underline{\textcolor{blue}{0.0753}} & \underline{\textcolor{blue}{0.057}} & \textbf{\textcolor{red}{83.34}} \\
      RAFT+PerVFI & \underline{\textcolor{blue}{27.16}}&     \textbf{\textcolor{red}{0.816}}&      \textbf{\textcolor{red}{0.0751}} &     \textbf{\textcolor{red}{0.056}}&      \underline{\textcolor{blue}{83.30}} \\
      \bottomrule
    \end{tabular}
  \end{adjustbox}
\end{table}

\begin{table}[tbp]
  \centering
  \caption{Comparison of different methods in terms of runtime, Multiply-ACcumulate operations Counting (MACs), and the number of parameters. The notation ``*PerVFI'' indicates that the optical flows are pre-obtained. ``GMFlow+PerVFI'' and ``RAFT+PerVFI'' refer to the usage of GMFlow~\cite{gmflow} and RAFT~\cite{raft} for optical flow estimation prior to interpolation. The evaluations are conducted on frames of size $512\times 512$ on a NVIDIA RTX 3090 GPU.}
  \label{tab:runtime}
  \begin{adjustbox}{max width=\linewidth}
  \begin{tabular}{lccc}
    \toprule
    Methods & Runtime (s) $\downarrow$ & MACs (G) $\downarrow$ & \#Params (M) $\downarrow$ \\
    \midrule
    EDSC~\cite{cheng2021multiple} & 0.077 & 71.826 & 8.945 \\
    XVFI~\cite{sim2021xvfi} & 0.067 & 70.725 & 5.577 \\
    RIFE~\cite{huang2020rife} & 0.037 & 52.247 & 2.278 \\
    EBME~\cite{Jin_2023_WACV} & 0.079 & 43.731 & 3.908 \\
    STMFNet~\cite{Danier_2022_CVPR} & 0.206 & 876.156 & 17.960 \\
    % EMA-VFI~\cite{zhang2023extracting} & 0.206 & 876.156 & 17.960 \\
    \midrule
    *PerVFI & 0.161 & 458.340 & 8.481 \\
    GMFlow+PerVFI & 0.193 & 523.758 & 13.161 \\
    RAFT+PerVFI & 0.204 & 836.591 & 13.739 \\
    \bottomrule
  \end{tabular}
  \end{adjustbox}
\end{table}

% \begin{figure}[tbp]
%     \centering
%     \begin{adjustbox}{max width=\textwidth}
%     \begin{tabular}{cccc|ccccc}
%       \toprule
%       Mask & Noise & Prior & Loss & PSNR & SSIM & LPIPS & FloLPIPS & VFIPS\\
%       \midrule
%       Binary & \ding{55} & \ding{51} & Bi-D. & 26.52 & 81.01 \\
%       Quasi-B. & \ding{55} & \ding{51} & Bi-D. & 26.71 & 81.24 \\
%       Quasi-B. & \ding{51} & \ding{55} & Bi-D. & 27.10 & 82.27 \\
%       Quasi-B. & \ding{51} & \ding{55} & L1 & 26.81 & 80.34 \\
%       Quasi-B. & \ding{51} & \ding{51} & L1 & 27.15 & 80.50 \\
%       Quasi-B. & \ding{51} & \ding{51} & NLL & 26.98 & 81.88 \\
%       Binary & \ding{51} & \ding{51} & Bi-D. & 26.69 & 81.25 \\
%       Adaptive & \ding{51} & \ding{51} & Bi-D. & \textbf{27.61} & 78.20 \\
%       \midrule
%       Quasi-B. & \ding{51} & \ding{51} & Bi-D. & 27.16 & \textbf{83.30} \\
%       \bottomrule
%     \end{tabular}
%     \end{adjustbox}
%     \captionof{table}{Ablation Experiment Results on DAVIS (480P) dataset~\cite{davis}.}
%     \label{tab:ablation}
% \end{figure}

% \begin{figure}[tbp]
%     \centering
%     \begin{adjustbox}{max width=\textwidth}
%     \begin{tabular}{cccc|ccccc}
%       \toprule
%       Mask & Noise & Prior & Loss & PSNR & SSIM & LPIPS & FloLPIPS & VFIPS\\
%       \midrule
%       Binary & \ding{55} & \ding{51} & Bi-D. & 26.52 & 81.01 \\
%       Quasi-B. & \ding{55} & \ding{51} & Bi-D. & 26.71 & 81.24 \\
%       Quasi-B. & \ding{51} & \ding{55} & Bi-D. & 27.10 & 82.27 \\
%       Quasi-B. & \ding{51} & \ding{55} & L1 & 26.81 & 80.34 \\
%       Quasi-B. & \ding{51} & \ding{51} & L1 & 27.15 & 80.50 \\
%       Quasi-B. & \ding{51} & \ding{51} & NLL & 26.98 & 81.88 \\
%       Binary & \ding{51} & \ding{51} & Bi-D. & 26.69 & 81.25 \\
%       Adaptive & \ding{51} & \ding{51} & Bi-D. & \textbf{27.61} & 78.20 \\
%       \midrule
%       Quasi-B. & \ding{51} & \ding{51} & Bi-D. & 27.16 & \textbf{83.30} \\
%       \bottomrule
%     \end{tabular}
%     \end{adjustbox}
%     \captionof{table}{Ablation Experiment Results on DAVIS (1080P) dataset~\cite{davis}.}
%     \label{tab:ablation}
% \end{figure}
